Understanding the Excess Bond Premium

We study the drivers of the Gilchrist and Zakraj\v{s}ek (2012) excess bond premium (EBP) through the lens of the news. The monthly attention the news pays to 180 topics (Bybee et al., 2024) captures up to 80% of the variation in the EBP, and this component of variation forecasts macroeconomic movements. Greater news attention to financial intermediaries and crises tends to drive up the EBP and portend macroeconomic downturns, while greater news attention to politics and science tends to drive down the EBP. Attention-based estimates of EBP largely drive out the forecast power of direct sentiment measures for macroeconomic fluctuations and predict the business cycle going back to the early 1900's. Overall, we attribute predictive variation about the EBP for macroeconomic movements to variation in news attention to financial intermediaries, crises, and politics.

==> tables/table2-12m.tex <==
\begin{tabular}{lccccc}
\hline\hline
 & EMP (SA) & UER & IPM & GDP & Recession \\
 & (1) & (2) & (3) & (4) & (5) \\
\cmidrule(lr){2-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6}
TS & 0.3381 & -0.1949 & 1.1746*** & 0.1378 & -0.645*** \\
 & (0.36) & (0.22) & (0.40) & (0.35) & (0.233) \\
RFF & -0.0832 & 0.1756* & 0.0165 & -0.0568 & 0.177 \\
 & (0.15) & (0.09) & (0.21) & (0.16) & (0.114) \\
$\tilde{\text{GZF}}$ & -1.1286*** & 0.6831*** & -2.5166*** & -1.2942*** & 0.883** \\
 & (0.27) & (0.19) & (0.86) & (0.49) & (0.357) \\
$\hat{\text{EBP}}$ & -1.6300*** & 0.7891*** & -1.5311 & -1.0960*** & 1.627*** \\
 & (0.23) & (0.13) & (0.99) & (0.39) & (0.317) \\
$R^2$ & 0.268 & 0.263 & 0.201 & 0.161 & 0.420 \\
$T$ & 427 & 427 & 427 & 142 & 427 \\
SHAP($\tilde{\text{GZF}}$) & 30.02 & 23.81 & 37.01 & 44.23 & 19.89 \\
SHAP($\hat{\text{EBP}}$) & 35.11 & 22.27 & 18.23 & 32.04 & 31.95 \\
\hline
\end{tabular}


==> tables/table2-slide.tex <==
\begin{tabular}{lccccc}
\hline\hline
 & EMP (SA) & UER & IPM & GDP & Recession \\
 & (1) & (2) & (3) & (4) & (5) \\
\cmidrule(lr){2-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6}
$\hat{\text{EBP}}$ & -2.740*** & 1.813*** & -6.823*** & -2.450*** & 1.669*** \\
 & (0.63) & (0.48) & (1.56) & (0.62) & (0.28) \\
$\hat{\text{EBP}}$-RES & -1.709*** & 1.282*** & -7.237*** & -2.622*** & 0.797** \\
 & (0.37) & (0.28) & (1.58) & (0.60) & (0.32) \\
GZF & -1.006** & 0.468* & -0.466 & -0.682 & 0.254 \\
 & (0.40) & (0.28) & (1.06) & (0.60) & (0.51) \\
 \\
$R^2$ & 0.162 & 0.145 & 0.262 & 0.183 & 0.372 \\
$T$ & 427 & 427 & 427 & 142 & 427 \\
SHAP(GZF) & 14.67 & 8.98 & 2.08 & 9.47 & 7.22 \\
SHAP($\hat{\text{EBP}}$) & 36.57 & 31.78 & 27.87 & 32.76 & 52.92 \\
SHAP($\hat{\text{EBP}}$-RES) & 20.24 & 19.95 & 26.24 & 30.70 & 19.67 \\
\hline
\end{tabular}


==> tables/table2.tex <==
\begin{tabular}{lccccc}
\hline\hline
 & EMP (SA) & UER & IPM & GDP & Recession \\
 & (1) & (2) & (3) & (4) & (5) \\
\cmidrule(lr){2-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6}
TS & 0.2957 & -0.2061 & 1.3963** & 0.1524 & -0.123 \\
 & (0.49) & (0.37) & (0.66) & (0.41) & (0.209) \\
RFF & -0.0014 & 0.1641 & -0.0072 & -0.0241 & 0.144 \\
 & (0.19) & (0.14) & (0.29) & (0.18) & (0.113) \\
$\tilde{\text{GZF}}$ & -1.4117*** & 0.9377*** & -4.2597*** & -1.8250*** & 0.584* \\
 & (0.20) & (0.17) & (1.18) & (0.52) & (0.305) \\
$\hat{\text{EBP}}$ & -2.4969*** & 1.5308*** & -4.1641*** & -1.8120*** & 1.479*** \\
 & (0.50) & (0.38) & (1.28) & (0.56) & (0.242) \\
$R^2$ & 0.162 & 0.142 & 0.213 & 0.167 & 0.366 \\
$T$ & 427 & 427 & 427 & 142 & 427 \\
SHAP($\tilde{\text{GZF}}$) & 28.95 & 21.86 & 34.09 & 41.67 & 21.69 \\
SHAP($\hat{\text{EBP}}$) & 41.45 & 28.90 & 26.98 & 35.39 & 48.91 \\
\hline
\end{tabular}


==> tables/table3_EBP_base_gpt_slides.tex <==
\begin{tabular}{llrr}
\toprule
 &  & Explained Variance & \multicolumn{1}{c}{$\hat{w}$} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-4}
\multirow[t]{4}{*}{Top Positive} & Crisis / Disasters & 9.97 & 60.2 \\
 & Financial Crisis & 6.22 & 69.6 \\
 & Negative Sentiment & 2.82 & 31.9 \\
 & Financial Intermediaries & 2.61 & 73.6 \\
\multirow[t]{7}{*}{Top Negative} & Politics & 28.16 & -48.6 \\
 & Other & 22.94 & -4.8 \\
 & Industry & 11.46 & -53.6 \\
 & Financial Markets / Economy & 11.31 & -26.2 \\
 & Positive Sentiment & 3.23 & -17.2 \\
 & Science / Technology & 0.79 & -10.3 \\
 & Economic Growth & 0.49 & -17.1 \\
\bottomrule
\end{tabular}


==> tables/table3_GZF_base_gpt_slides.tex <==
\begin{tabular}{llrr}
\toprule
 &  & Explained Variance & \multicolumn{1}{c}{$\hat{w}$} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-4}
\multirow[t]{5}{*}{Top Positive} & Financial Markets / Economy & 30.47 & 19.8 \\
 & Crisis / Disasters & 7.14 & 44.5 \\
 & Negative Sentiment & 6.90 & 0.1 \\
 & Financial Intermediaries & 4.09 & 36.1 \\
 & Financial Crisis & 4.09 & 47.3 \\
\multirow[t]{6}{*}{Top Negative} & Other & 19.11 & -38.9 \\
 & Politics & 13.34 & -0.6 \\
 & Industry & 13.02 & -20.8 \\
 & Science / Technology & 1.83 & -6.9 \\
 & Positive Sentiment & 0.02 & -0.7 \\
 & Economic Growth & 0.01 & -2.1 \\
\bottomrule
\end{tabular}


==> tables/table4-12m.tex <==
\begin{tabular}{lccccc}
\hline\hline
 & EMP (SA) & UER & IPM & GDP & Recession \\
 & (1) & (2) & (3) & (4) & (5) \\
\cmidrule(lr){2-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6}
TS & 0.3686 & -0.2341 & 1.6557*** & 0.2020 & -0.531** \\
 & (0.39) & (0.24) & (0.41) & (0.40) & (0.231) \\
RFF & 0.0848 & 0.0677 & 0.5883** & -0.0004 & 0.015 \\
 & (0.18) & (0.12) & (0.27) & (0.22) & (0.126) \\
$\tilde{\text{GZF}}$ & -0.2641 & 0.1695 & -0.9178 & -0.5600 & -0.206 \\
 & (0.38) & (0.22) & (0.93) & (0.52) & (0.425) \\
$\hat{\text{EBP}}$-FI & -4.0679** & 2.2157** & -10.3406*** & -3.1210 & 1.321 \\
 & (1.61) & (1.01) & (3.49) & (2.23) & (1.355) \\
$\hat{\text{EBP}}$-FCRIS & -1.1488 & 0.5339 & 1.6982 & -2.4682 & 1.176 \\
 & (0.90) & (0.53) & (3.08) & (2.37) & (1.202) \\
$\hat{\text{EBP}}$-RES & -1.6079*** & 0.9377*** & -3.0988*** & -0.9987** & 1.828*** \\
 & (0.35) & (0.19) & (0.89) & (0.40) & (0.421) \\
$R^2$ & 0.260 & 0.281 & 0.302 & 0.168 & 0.394 \\
$T$ & 427 & 427 & 427 & 142 & 427 \\
\hline
\end{tabular}


==> tables/table4.tex <==
\begin{tabular}{lccccc}
\hline\hline
 & EMP (SA) & UER & IPM & GDP & Recession \\
 & (1) & (2) & (3) & (4) & (5) \\
\cmidrule(lr){2-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6}
TS & 0.1892 & -0.1522 & 1.9777*** & 0.1956 & -0.128 \\
 & (0.49) & (0.37) & (0.69) & (0.45) & (0.165) \\
RFF & 0.1754 & 0.0370 & 0.7340* & 0.1231 & -0.028 \\
 & (0.28) & (0.21) & (0.39) & (0.24) & (0.109) \\
$\tilde{\text{GZF}}$ & -0.0633 & -0.0026 & -0.8298 & -0.4574 & -0.330 \\
 & (0.42) & (0.30) & (0.91) & (0.47) & (0.360) \\
$\hat{\text{EBP}}$-FI & -3.0721*** & 1.8258*** & -16.5301*** & -3.5507** & 2.955*** \\
 & (1.03) & (0.71) & (3.80) & (1.74) & (0.897) \\
$\hat{\text{EBP}}$-FCRIS & -2.7426*** & 1.8532** & -4.6805 & -3.3519 & 1.420 \\
 & (1.03) & (0.77) & (3.33) & (2.28) & (0.903) \\
$\hat{\text{EBP}}$-RES & -2.4963*** & 1.7132*** & -6.0930*** & -2.1496*** & 1.526*** \\
 & (0.84) & (0.61) & (1.49) & (0.56) & (0.356) \\
$R^2$ & 0.137 & 0.133 & 0.287 & 0.178 & 0.345 \\
$T$ & 427 & 427 & 427 & 142 & 427 \\
\hline
\end{tabular}


==> tables/table7.tex <==
\begin{tabular}{lcccccc}
\hline\hline
 & \multicolumn{3}{c}{Forecast horizon: 3 months} & \multicolumn{3}{c}{Forecast horizon: 12 months} \\
 & CPI & UER & IPM & CPI & UER & IPM \\
 & (1) & (2) & (3) & (4) & (5) & (6) \\
 \cmidrule(lr){2-4} \cmidrule(lr){5-7}
$\hat{\text{EBP}}$ & -0.6168 & 1.9394** & -3.1097 & -1.1908* & 2.1235*** & -3.6490 \\
 & (0.78) & (0.83) & (3.63) & (0.64) & (0.69) & (3.23) \\
$R^2$ & 0.365 & 0.162 & 0.082 & 0.237 & 0.151 & 0.032 \\
$T$ & 696 & 521 & 645 & 1002 & 521 & 645 \\
SHAP($\hat{\text{EBP}}$) & 4.82 & 30.94 & 13.72 & 14.88 & 47.76 & 31.25 \\
\hline
\end{tabular}


==> tables/table7_bkmx_decomp.tex <==
\begin{tabular}{lcccccc}
\hline\hline
 & \multicolumn{3}{c}{Forecast horizon: 3 months} & \multicolumn{3}{c}{Forecast horizon: 12 months} \\
 & CPI & UER & IPM & CPI & UER & IPM \\
 & (1) & (2) & (3) & (4) & (5) & (6) \\
 \cmidrule(lr){2-4} \cmidrule(lr){5-7}
BAA-Yield & -0.8736*** & 0.3361 & -0.6654 & -0.8241** & 0.0778 & 0.5855 \\
 & (0.28) & (0.29) & (1.43) & (0.33) & (0.26) & (1.13) \\
TBill-Yield & 0.1511 & 0.3214 & -0.9240 & 0.1961 & 0.5032** & -1.4967 \\
 & (0.25) & (0.23) & (1.14) & (0.32) & (0.23) & (1.13) \\
$\hat{\text{EBP}}$-ANNO & -0.8567 & -1.6093 & 6.0393 & -0.5380 & -0.3396 & 0.2326 \\
 & (1.60) & (1.38) & (6.43) & (1.77) & (1.40) & (6.82) \\
$\hat{\text{EBP}}$-EARN & -39.9904*** & 33.1877** & -96.8474*** & -34.0494*** & 31.8875*** & -43.5463 \\
 & (9.62) & (15.21) & (37.27) & (10.12) & (8.56) & (31.25) \\
$\hat{\text{EBP}}$-GROWTH & -2.9099* & 3.8230** & -14.0416 & -3.6408** & 0.8910 & 5.5812 \\
 & (1.69) & (1.63) & (8.98) & (1.49) & (1.23) & (7.20) \\
$\hat{\text{EBP}}$-FCRIS & 16.7253 & 16.0161 & 51.2938 & 16.8526* & 3.6290 & 13.7892 \\
 & (12.57) & (12.09) & (62.93) & (9.15) & (6.77) & (25.28) \\
$\hat{\text{EBP}}$-FI & 0.5031 & -3.6054 & 38.2797** & 5.9431 & -10.0643*** & 49.7389*** \\
 & (4.19) & (3.82) & (18.45) & (4.76) & (2.77) & (14.84) \\
$\hat{\text{EBP}}$-MKT & -4.3760 & 1.7475 & 13.8161 & -2.5591 & 7.7000* & -11.4931 \\
 & (5.12) & (6.75) & (19.57) & (5.66) & (4.09) & (20.00) \\
$\hat{\text{EBP}}$-IND & 3.2595 & 11.1168** & -48.7438** & -7.7727 & 12.1866*** & -39.0371** \\
 & (4.71) & (4.56) & (22.06) & (4.81) & (3.79) & (16.89) \\
$\hat{\text{EBP}}$-ITNREL & -5.2814 & 0.4159 & 15.2510 & -8.8342*** & 0.3694 & -8.0977 \\
 & (3.32) & (3.10) & (17.22) & (3.18) & (2.59) & (14.02) \\
$\hat{\text{EBP}}$-NTLPLC & -2.5317 & 3.6524* & -9.2695 & -0.2840 & 2.1186 & 0.9451 \\
 & (2.09) & (1.94) & (7.17) & (2.74) & (1.33) & (4.99) \\
$\hat{\text{EBP}}$-OILMINE & 16.6237 & -19.9218** & 73.4036** & 1.2508 & 3.0504 & 14.9394 \\
 & (13.06) & (8.62) & (33.53) & (8.52) & (10.35) & (36.17) \\
$\hat{\text{EBP}}$-SCIART & -1.1717 & 4.4557** & 3.9889 & -4.4416* & 3.9711** & -4.5235 \\
 & (2.18) & (2.18) & (8.10) & (2.36) & (1.57) & (6.09) \\
$\hat{\text{EBP}}$-TECH & 18.6808** & -11.0848 & 54.6638 & 12.1942 & -7.8299 & 21.3362 \\
 & (8.65) & (7.10) & (36.93) & (8.55) & (4.88) & (23.40) \\
$R^2$ & 0.383 & 0.239 & 0.135 & 0.360 & 0.370 & 0.145 \\
$T$ & 648 & 521 & 645 & 648 & 521 & 645 \\
\hline
\end{tabular}


==> tables/table7b.tex <==
\begin{tabular}{lcccc}
\hline\hline
 & \multicolumn{2}{c}{Forecast horizon: 1 quarter} & \multicolumn{2}{c}{Forecast horizon: 4 quarters} \\
 & GDP & NFI & GDP & NFI \\
 & (1) & (2) & (3) & (4)\\
 \cmidrule(lr){2-3} \cmidrule(lr){4-5}
$\hat{\text{EBP}}$ & -2.2248* & -9.6695*** & -1.6748** & -5.8808** \\
 & (1.14) & (2.61) & (0.85) & (2.51) \\
$R^2$ & 0.176 & 0.348 & 0.049 & 0.179 \\
$T$ & 104 & 104 & 104 & 104 \\
SHAP($\hat{\text{EBP}}$) & 34.19 & 24.42 & 42.65 & 27.93 \\
\hline
\end{tabular}


==> tables/table7b_bkmx_decomp.tex <==
\begin{tabular}{lcccc}
\hline\hline
 & \multicolumn{2}{c}{Forecast horizon: 1 quarter} & \multicolumn{2}{c}{Forecast horizon: 4 quarters} \\
 & GDP & NFI & GDP & NFI \\
 & (1) & (2) & (3) & (4)\\
 \cmidrule(lr){2-3} \cmidrule(lr){4-5}
BAA-Yield & -0.0668 & -0.8641 & 0.1937 & 0.5041 \\
 & (0.41) & (1.09) & (0.37) & (0.68) \\
TBill-Yield & -0.7303** & -0.5940 & -0.9757*** & -2.6755*** \\
 & (0.35) & (0.81) & (0.28) & (0.49) \\
$\hat{\text{EBP}}$-ANNO & -5.0747 & -6.8150 & -3.6523 & 2.3681 \\
 & (3.82) & (9.72) & (2.78) & (7.04) \\
$\hat{\text{EBP}}$-EAR$T$ & -20.4994 & -70.3207 & -17.5682 & -134.1961*** \\
 & (26.21) & (70.60) & (20.10) & (44.57) \\
$\hat{\text{EBP}}$-GROWTH & -6.5848** & -30.1598*** & -1.9153 & -12.9172*** \\
 & (3.27) & (8.01) & (1.47) & (4.02) \\
$\hat{\text{EBP}}$-FCRIS & 3.2945 & -3.7572 & -0.6237 & 16.5782 \\
 & (23.70) & (75.91) & (20.18) & (36.17) \\
$\hat{\text{EBP}}$-FI & 7.0688 & 28.7873 & 8.0591 & 32.1196** \\
 & (7.18) & (19.90) & (5.91) & (14.11) \\
$\hat{\text{EBP}}$-MKT & -8.9589 & -16.9948 & -10.4569 & -31.4309** \\
 & (9.27) & (24.63) & (7.45) & (14.76) \\
$\hat{\text{EBP}}$-IND & 4.6282 & -10.3492 & 4.2573 & -25.7920** \\
 & (7.51) & (21.79) & (3.79) & (11.02) \\
$\hat{\text{EBP}}$-ITNREL & -5.9047 & -19.4849** & -2.8965 & -21.0445*** \\
 & (4.53) & (9.42) & (2.45) & (6.26) \\
$\hat{\text{EBP}}$-NTLPLC & -1.1410 & -6.1083 & -4.7306 & -10.0414 \\
 & (4.38) & (10.39) & (3.10) & (8.23) \\
$\hat{\text{EBP}}$-OILMINE & 6.8571 & -33.9291 & -0.2884 & -17.7966 \\
 & (17.87) & (50.62) & (16.43) & (36.32) \\
$\hat{\text{EBP}}$-SCIART & -0.4608 & 1.5032 & -0.5470 & -5.5724 \\
 & (2.95) & (9.65) & (2.45) & (5.81) \\
$\hat{\text{EBP}}$-TECH & 19.3379 & 93.3930* & 0.1820 & 50.5850* \\
 & (18.87) & (50.10) & (10.79) & (29.06) \\
$R^2$ & 0.204 & 0.386 & 0.160 & 0.328 \\
$T$ & 104 & 104 & 104 & 104 \\
\hline
\end{tabular}


==> tables/table9-12m.tex <==
\begin{tabular}{lccccc}
\hline\hline
 & EMP (SA) & UER & IPM & GDP & Recession \\
 & (1) & (2) & (3) & (4) & (5) \\
\cmidrule(lr){2-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6}
TS & 0.2841 & -0.1201 & 1.0550** & 0.1245 & -0.722** \\
 & (0.41) & (0.26) & (0.46) & (0.36) & (0.283) \\
RFF & -0.0597 & 0.1448* & 0.2435 & 0.1788 & 0.104 \\
 & (0.15) & (0.09) & (0.21) & (0.15) & (0.114) \\
GZF-IG & -1.6064** & 0.5841 & -1.1204 & 0.7377 & 0.593 \\
 & (0.67) & (0.38) & (1.84) & (0.69) & (0.908) \\
$\hat{\text{EBP-IG}}$ & -2.2763*** & 1.4703*** & -4.4785*** & -3.5232*** & 3.625*** \\
 & (0.49) & (0.27) & (1.58) & (0.90) & (0.762) \\
$\hat{\text{EBP-IG}}$-RES & -1.7414*** & 1.3167*** & -5.5839*** & -2.8795*** & 2.347*** \\
 & (0.49) & (0.33) & (1.07) & (0.71) & (0.693) \\
$R^2$ & 0.254 & 0.276 & 0.234 & 0.243 & 0.484 \\
$T$ & 408 & 408 & 408 & 136 & 408 \\
SHAP(GZF-IG) & 21.58 & 10.57 & 6.12 & 7.25 & 5.83 \\
SHAP($\hat{\text{EBP-IG}}$) & 29.96 & 26.08 & 23.98 & 35.49 & 37.81 \\
SHAP($\hat{\text{EBP-IG}}$-RES) & 21.77 & 22.18 & 28.40 & 29.30 & 21.71 \\
\hline
\end{tabular}


==> tables/table9b-12m.tex <==
\begin{tabular}{lccccc}
\hline\hline
 & EMP (SA) & UER & IPM & GDP & Recession \\
 & (1) & (2) & (3) & (4) & (5) \\
\cmidrule(lr){2-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6}
TS & 0.3498 & -0.1852 & 1.3119*** & 0.2518 & -0.879*** \\
 & (0.39) & (0.25) & (0.48) & (0.38) & (0.213) \\
RFF & -0.0078 & 0.1164 & 0.2055 & 0.1320 & 0.052 \\
 & (0.19) & (0.12) & (0.28) & (0.22) & (0.108) \\
GZF-HY & -0.2737 & 0.0583 & -0.4580 & -0.0123 & -0.099 \\
 & (0.33) & (0.18) & (0.78) & (0.38) & (0.330) \\
$\hat{\text{EBP-HY}}$ & -1.4548*** & 0.8553*** & -1.4436 & -2.0621*** & 2.350*** \\
 & (0.28) & (0.18) & (1.21) & (0.64) & (0.379) \\
$\hat{\text{EBP-HY}}$-RES & -0.7164*** & 0.4090*** & -1.2650*** & -0.5513*** & 0.817*** \\
 & (0.16) & (0.09) & (0.32) & (0.21) & (0.216) \\
$R^2$ & 0.248 & 0.240 & 0.160 & 0.135 & 0.496 \\
$T$ & 408 & 408 & 408 & 136 & 408 \\
SHAP(GZF-HY) & 13.50 & 3.93 & 9.87 & 0.52 & 3.10 \\
SHAP($\hat{\text{EBP-HY}}$) & 23.85 & 19.17 & 10.34 & 30.15 & 28.27 \\
SHAP($\hat{\text{EBP-HY}}$-RES) & 31.78 & 24.80 & 24.53 & 21.23 & 28.76 \\
\hline
\end{tabular}

